Solving Fredholm Integral Equations of the First Kind via Wasserstein Gradient Flows

Solving Fredholm equations of the first kind is crucial in many areas of the applied sciences. In this work we adopt a probabilistic and variational point of view by considering a minimization problem in the space of probability measures with an entropic regularization. Contrary to classical approaches which discretize the domain of the solutions, we introduce an algorithm to asymptotically sample from the unique solution of the regularized minimization problem. As a result our estimators do not depend on any underlying grid and have better scalability properties than most existing methods. Our algorithm is based on a particle approximation of the solution of a McKean--Vlasov stochastic differential equation associated with the Wasserstein gradient flow of our variational formulation. We prove the convergence towards a minimizer and provide practical guidelines for its numerical implementation. Finally, our method is compared with other approaches on several examples including density deconvolution and epidemiology.

==> gradient_flow.tex <==
\subsection{Basics on Wasserstein gradient flows and subdifferential of $\Gun_\alpha^\eta$}
\label{app:subdifferential}
In this section we recall basics results on gradient flows in Wasserstein spaces
and provide a slight extension of the classical variational formula. We refer to \cite{ambrosio2008gradient} for further details.  We denote by $\rmL^2(\rset^d, \nu)$
the set of square integrable functions w.r.t. a measure $\nu$, % , \ie \ 
% $\int_{\rset^d} \varphi(x)^2 \rmd \nu(x)<\infty$,
by $\rmc_c^\infty(\rset^d)$ the set of infinitely
many times differentiable functions with compact support and by $\rmW^{1,1}_{\mathrm{loc}}(\rset^d)$ the set of functions which are in $\rmW^{1,1}_{\mathrm{loc}}(\msx)$ for all compact sets $\msx\subset \rset^d$, where $\rmW^{1,1}_{\mathrm{loc}}(\msx)$ denotes the Sobolev space of functions whose zero-th and first derivative are bounded in $\rmL^1$.  For any
$\nu\in\Pens(\rset^d)$ and $t: \ \rset^d \to \rset^d$ measurable, we denote by
$t_{\#}\nu$ the push-forward measure, $t_{\#}\nu(A)=\nu(t^{-1}(A))$ for all
$A\in\mcb {\rset^d}$.  We start by recalling the definition of the
subdifferentiability in Wasserstein spaces, see \cite[Definition
10.1.1]{ambrosio2008gradient}. We denote $\Pens_{2}^r(\rset^d)$ the space of
probability distributions in $\Pens_2(\rset^d)$ which are absolutely continuous
w.r.t the Lebesgue measure.

\begin{definition}[Fr\'echet subdifferential]
  Let $\Phi: \ \Pens_2(\rset^d) \to \ooint{-\infty, +\infty}$. Let
  $\pi \in \Pens_{2}^r(\rset^d)$, then
  $\xi \in \rmL^2(\rset^d, \pi)$ belongs to the strong Fr\'{e}chet
    subdifferential $\partial_{\rms} \Phi(\pi)$ of $\Phi$ at $\pi$ if for any $t \in \rmL^2(\rset^d, \pi)$
    \begin{equation}
      \textstyle{
        \liminf_{t \to \Id}\left. \defEns{\Phi(t_\# \pi) - \Phi(\pi) - \int_{\rset^d} \langle \xi(x), t(x) - x \rangle \rmd \pi(x)}\middle/ \norm{t - \Id}_{\rmL^2(\rset^d, \pi)} \right. = 0.
        }
  \end{equation}
\end{definition}

The following lemma is a specific case of the chain-rule formula.

\begin{lemma}
  \label{lemma:chain_rule}
  Let $g \in \rmc^1(\rset, \rset)$ be Lipschitz, convex and lower-bounded. For any
  $y \in \rset^p$, let $\Lun : \ \Pens_2(\rset^d) \times \rset^p \to \rset$,
  $\pi \in \Pens_2(\rset^d)$, $\mu \in \Pens_2(\rset^p)$ and
  $\xi \in \rmL^2(\rset^d \times \rset^p, \pi \otimes \mu)$ such that for any
  $y \in \rset^p$ and $\pi \in \Pens_{2}^r(\rset^d)$,
  $\xi(\pi, y) \in \partial_{\rms} \Lun(\pi, y)$ and
  $-\xi(\pi, y) \in \partial_{\rms} (-\Lun)(\pi, y)$.
  In addition, assume
  that there exists $h \in \rmL^1(\rset^p, \mu)$ such that for any
  $\pi_1, \pi_2 \in \Pens_2(\rset^d)$ and $y \in \rset^p$ we have
  \begin{equation}
    \abs{\Lun(\pi_1, y) - \Lun(\pi_2, y)} \leq h(y) \wassersteinD[2](\pi_1, \pi_2). 
  \end{equation}
Let $\Mun$ be given for any $\pi \in \Pens(\rset^d)$ by
\begin{equation}
  \textstyle{
    \Mun(\pi) = \int_{\rset^p} g(\Lun(\pi, y)) \rmd \mu(y).
    }
  \end{equation}  
  Then, we have that $\partial_{\rms} \Mun(\pi) \neq \emptyset$ and
  $\defEnsLigne{x \mapsto \int_{\rset^p} g'(\Lun(\pi, y)) \xi(\cdot, y) \rmd
    \mu(y)} \in \partial_{\mathrm{s}} \Mun(\pi)$.
\end{lemma}

\begin{proof}
  Let $\pi \in \Pens(\rset^d)$, $t \in \rmL^2(\rset^d, \pi)$ and $y \in \rset^d$.  Since $g$ is convex we have
  \begin{equation}
    g(\Lun(t_\# \pi, y)) - g(\Lun(\pi, y)) \geq g'(\Lun(\pi, y)) (\Lun(t_\# \pi, y) - \Lun(\pi, y)). 
  \end{equation}
  We have 
  \begin{multline}
    \label{eq:inter_convx}
    \textstyle{g(\Lun(t_\# \pi, y)) - g(\Lun(\pi, y)) - g'(\Lun(\pi, y)) \int_{\rset^d} \langle \xi(x,y), t(x) - x \rangle \rmd \pi(x)} \\
    \textstyle{\geq g'(\Lun(\pi, y)) \parenthese{\Lun(t_\# \pi, y) - \Lun(\pi, y) - \int_{\rset^d} \langle \xi(x, y), t(x) - x \rangle \rmd \pi(x) }.}
  \end{multline}
  In addition, using that $\xi(\pi, y) \in \partial_{\rms} \Lun(\pi, y)$ and
  $-\xi(\pi, y) \in \partial_{\rms} (-\Lun)(\pi, y)$ we have
  \begin{align}
    \textstyle{
    \liminf_{t \to \Id} \parenthese{\Lun(t_\# \pi, y) - \Lun(\pi, y) - \int_{\rset^d} \langle \xi(x, y), t(x) - x \rangle \rmd \pi(x) } / \normLigne{t - \Id}_2  \geq 0,} \\
    \textstyle{\limsup_{t \to \Id} \parenthese{\Lun(t_\# \pi, y) - \Lun(\pi, y) - \int_{\rset^d} \langle \xi(x, y), t(x) - x \rangle \rmd \pi(x) } / \normLigne{t - \Id}_2  \leq 0.}
  \end{align}
  Hence, we have
  \begin{equation}
    \textstyle{\lim_{t \to \Id} \parenthese{\Lun(t_\# \pi, y) - \Lun(\pi, y) - \int_{\rset^d} \langle \xi(x, y), t(x) - x \rangle \rmd \pi(x) } / \normLigne{t - \Id}_2  = 0.}
  \end{equation}
  We also have that
\begin{align}
  &\textstyle{\abs{\Lun(t_\# \pi, y) - \Lun(\pi, y) - \int_{\rset^d} \langle \xi(x, y), t(x) - x \rangle \rmd \pi(x) } / \normLigne{t - \Id}_2 }\\
  &\qquad\qquad\qquad\textstyle{\leq h(y) + \int_{\rset^d} \norm{\xi(x, y)} \rmd \pi(x). }
\end{align}
We conclude upon using this result, the fact that $g$ is Lipschitz,
\eqref{eq:inter_convx} and the dominated convergence theorem.
\end{proof}

We are now ready to derive the subdifferential of $\Gun_{\alpha}^{\eta}$ for any
$\eta > 0$.

\begin{lemma}[Strong subdifferential of $\Gun^{\eta}$]
  \label{lemma:subdiff_g_eta}
  Assume \tup{\Cref{assum:general_kker}}. Then for any
  $\pi \in \Pens_{2}^r(\rset^d)$ and $\eta > 0$, we have that 
  $\partial_{\rms} \Gun^\eta(\pi) \neq \emptyset$ and
  \begin{equation}
    \textstyle{
      \defEnsLigne{x \mapsto \int_{\rset^p} (\eta + \pi[\kker(x, y)])^{-1} \nabla_1
        \kker(x, y) \rmd \mu(y)} \in \partial_{\rms} \Gun^\eta(\pi). }
  \end{equation}
 
 
\end{lemma}

\begin{proof}
  First, using that $\normLigne{\rmd^2 \kker} \leq \Mtt$ we get that for any $x_1, x_2 \in \rset^d$, $y\in\rset^p$
  \begin{equation}
    \label{eq:lambda_cvx}
    \kker(x_2, y) \geq \kker(x_1, y) + \langle \nabla_1 \kker(x_1, y), x_2 -x_1 \rangle - \Mtt \norm{x_1 - x_2}^2.
  \end{equation}
  Let $\Lun: \ \Pens_2(\rset^d) \times \rset^p \to \coint{0, +\infty}$ given for
  any $\pi \in \Pens_2(\rset^d)$ and $y \in \rset^p$ by
  \begin{equation}
    \textstyle{
      \Lun(\pi, y) = \int_{\rset^d} \kker(x, y) \rmd \pi(x).
      }
  \end{equation}
  Using~\eqref{eq:lambda_cvx} and \cite[Proposition
  10.4.2]{ambrosio2008gradient} we get that for any $y \in \rset^p$ and
  $\pi \in \Pens_2(\rset^d)$,
  $\partial_{\rms} \Lun(\pi, y) = \{\partial_1 \kker(\cdot, y)\}$.  Since there
  exists $\norm{\partial_1 \kker}_{\infty} \leq \Mtt < +\infty$ we get that for
  any $\pi_1, \pi_2 \in \Pens_2(\rset^d)$ and $y \in \rset^p$
  \begin{equation}
    \label{eq:lip}
    \abs{\Lun(\pi_1, y) - \Lun(\pi_2, y)} \leq \Mtt \wassersteinD[2](\pi_1, \pi_2). 
  \end{equation}
  In addition, let $g : \ \ooint{0, +\infty} \to \rset$ given for any $t \geq 0$
  by $g(t) = -\log(t + \eta)$. Using that $g$ is convex,~\eqref{eq:lip} and that
  $\norm{\partial_1 \kker}_{\infty} \leq \Mtt < +\infty$ in \Cref{lemma:chain_rule}, we
  get that for any $\pi \in \Pens_2(\rset^d)$,
  $\partial_{\rms} \Gun^\eta(\pi) \neq \emptyset$ and
  $\defEnsLigne{x \mapsto \int_{\rset^d} (\eta + \pi[\kker(x, y)])^{-1} \nabla_1
    \kker(x, y) \rmd \mu(y)} \in \partial_{\rms} \Gun^\eta(\pi)$.
\end{proof}

Let $\Hun: \ \Pens(\rset^d) \to \ccint{0, +\infty}$ be defined for any
$\pi \in \Pens(\rset^d)$ by $\Hun(\pi) =
\KL{\pi}{\pi_0}$. \Cref{lemma:relative_entropy_sub} is a restatement of
\cite[Theorem 10.4.9]{ambrosio2008gradient}.

\begin{lemma}[Strong subdifferential of $\KL{\pi}{\pi_0}$]
  \label{lemma:relative_entropy_sub}
  Assume that 
  $\pi_0$
  admits a density, also denoted $\pi_0$, w.r.t. the Lebesgue measure such that for any $x \in \rset^d$,
  $\pi_0(x) \propto \exp[-U(x)]$ for some convex $U:\rset^d\to\rset$.
  Let $\pi \in \Pens_{2}^r(\rset^d)$
  such that $\Hun(\pi) < +\infty$ and
  $(\rmd \pi / \rmd \pi_0) \in \rmW^{1,1}_{\mathrm{loc}}(\rset^d, \ooint{0, +\infty})$. Then,
 \begin{align}
 \partial_{\rms} \Hun(\pi) = \defEns{x \mapsto \nabla \log(\rmd \pi / \rmd \pi_0)(x)}.
 \end{align}
  
\end{lemma}

Combining these two lemmas we are now ready to derive the subdifferential of
$\Gun_{\eta}^\alpha$ given by~\eqref{eq:G_eta} as well as one associated
Wasserstein gradient flow.

\begin{proposition}[Gradient flow]
\label{prop:total_subdifferential}
  Assume \tup{\Cref{assum:general_kker}} and that
  $\pi_0$
  admits a density, also denoted $\pi_0$, w.r.t. the Lebesgue measure such that for any $x \in \rset^d$,
  $\pi_0(x) \propto \exp[-U(x)]$ for some convex $U:\rset^d\to\rset$.
   Let $\pi \in \Pens_{2}^r(\rset^d)$ be
  such that $\KL{\pi}{\pi_0} < +\infty$ and
  $(\rmd \pi / \rmd \pi_0) \in \rmW^{1,1}_{\mathrm{loc}}(\rset^d, \ooint{0,
    +\infty})$. Then for any $\alpha, \eta > 0$
  \begin{equation}
    \textstyle{
   \defEns{x \mapsto \int_{\rset^p} (\eta + \pi[\kker(x, y)])^{-1} \nabla_1
    \kker(x, y) \rmd \mu(y) + \alpha \nabla \log(\rmd
    \pi / \rmd \pi_0)(x)} \in \partial_{\rms} \Gun_{\alpha}^\eta(\pi). }
  \end{equation}
  In addition, if $U \in \rmc^1(\rset^d, \rset)$ and there exists
  $(\pi_t)_{t \geq 0}$ such that for any $t \in \ooint{0, +\infty}$,
  $\rmd \pi_t / \rmd \Leb \in \rmc^1(\rset^d, \rset)$, and for any $\varphi \in \rmc_c^\infty(\rset^d)$
  \begin{multline}
    \textstyle{\int_{\rset} \varphi(x) \rmd \pi_t(x) - \int_{\rset} \varphi(x) \rmd
    \pi_0(x)} \\= \textstyle{\int_0^t \int_{\rset^d} \left[  -\int_{\rset^d} \defEns{ \left. \langle
      \nabla_1 \kker(x,y), \nabla \varphi(x) \rangle \middle/ \parenthese{\int_{\rset^d} \kker(x,
      y) \rmd \pi_s(x) + \eta}} \rmd \mu(y) \right. \right.} \\ \textstyle{\left. - \alpha \langle \nabla U(x), \nabla
      \varphi(x) \rangle + \alpha \Delta \varphi(x) \vphantom{\int_{\rset^d}}\right] \rmd \pi_s(x),}
  \end{multline}
  then $(\pi_t)_{t \geq 0}$ is a Wasserstein gradient flow associated with $\Gun_{\alpha}^\eta$.
\end{proposition}

\begin{proof}
  The first part of the proof is a straightforward application of
  \Cref{lemma:subdiff_g_eta} and \Cref{lemma:relative_entropy_sub}. The second
  part of the proof follows from the definition of a Wasserstein gradient flow
  \cite[Definition 11.1.1]{ambrosio2008gradient}.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> prop10_continuous_time.tex <==
\subsection{Stability of continuous time process}
\label{app:prop10_continuous_time}
\begin{proposition}
\label{prop:approx_mu_continuous_time}
Assume \tup{\rref{assum:general_kker}}, \rref{assum:lip_U}. Let
$\eta, \alpha > 0$. For any $N,M \in \nsets$, let $(\bfX_t^{1,N})_{t \geq 0}$
and $(\bfX_t^{1,N,M})_{t \geq 0}$ be the solution of \eqref{eq:particle} and
\eqref{eq:particle_M} respectively, with initial condition
$\bfX_0^{1:N} \in \Pens_1((\rset^d)^N)$ such that $\{\bfX_0^{k,N}\}_{k=1}^N$ is
exchangeable and $\{\bfX_0^{k,N}\}_{k=1}^N = \{\bfX_0^{k,N,M}\}_{k=1}^N$. Then
for any $T \geq 0$ there exists $C_T \geq 0$  such that for any $M, N \in \nsets$ and $\ell \in \{1, \dots, N\}$
  \begin{equation}
    \textstyle{
      \expeLigne{\sup_{t \in \ccint{0,T}} \normLigne{\bfX_t^{\ell,N}- \bfX_t^{\ell,N, M}}} \leq C_T M^{-1/2} \eqsp .
      }
  \end{equation}
\end{proposition}
\begin{proof}
The proofs is identical to that of \Cref{prop:approx_mu} with the discrete recursion replaced by an application of Gr\"{o}nwall's lemmma. Let $M, N \in \nsets$ and $\alpha, \eta > 0$. 
For any $k \in \{1, \dots, M\}$, $x_1 \in \rset^d$ and
$\nu_1 \in \Pens_1(\rset^d)$ let
$A_k = \tilde{b}_\eta(x_1, \nu_1, y^{k,M}) - \int_{\rset^p} \tilde{b}_\eta(x_1,
\nu_1, y) \rmd \mu(y)$. Then $\{A_k\}_{k=1}^M$ satisfies \eqref{eq:cond_AK} with
$C = \Mtt/\eta$. 

Combining this result, \eqref{eq:bound_bound},
\eqref{eq:intermezzo_duo} and that for any $t \geq 0$,
$\{\bfX_t^{k,N} - \bfX_t^{k,N,M}\}_{k=1}^N$ is exchangeable, we have that for
any $t \geq 0$,
\begin{align}
  &\expeLigne{\textstyle{\normLigne{b(\bfX_t^{1,N}, \bflambda_t^{N}) - b^M(\bfX_t^{1,N,M},\bflambda_t^{N,M})}}} \\
  &\qquad \textstyle{\leq ((\Mtt/\eta)(1 + (1/\eta)) + \Ltt)(1 + \Mtt) \parentheseLigne{ \expeLigne{\normLigne{\bfX_t^{1,N} - \bfX_t^{1,N,M}}} + (1/N) \sum_{k=1}^N \expeLigne{\normLigne{\bfX_t^{k,N} - \bfX_t^{k,N,M}}}}} \\
  & \qquad \qquad  \textstyle{+ \expeLigne{\normLigne{(1/M) \sum_{j=1}^M \{ \tilde{b}_\eta(\bfX_t^{1,N,M}, \bflambda_t^{N,M}, y^{j,M}) - \int_{\rset^p} \tilde{b}_\eta(\bfX_t^{1,N,M}, \bflambda_t^{N,M}, y) \rmd \mu(y)\}}}} \\
  &\qquad \textstyle{\leq 2((\Mtt/\eta)(1 + (1/\eta)) + \Ltt)(1 + \Mtt) \expeLigne{\normLigne{\bfX_t^{1,N} - \bfX_t^{1,N,M}}}} + (\Mtt/(M\eta))^{1/2}     \eqsp .
\end{align}
Using this result, we have for any $t \geq 0$
\begin{align}
  &\textstyle{ \expeLigne{\sup_{s \in \ccint{0,t}} \normLigne{\bfX_s^{1,N} - \bfX_s^{1,N,M}}} }\\
  & \qquad \qquad \qquad\textstyle{\leq 2((\Mtt/\eta)(1 + (1/\eta)) + \Ltt)(1 + \Mtt) \int_0^t \expeLigne{\sup_{u \in \ccint{0,s}} \normLigne{\bfX_u^{1,N} - \bfX_u^{1,N,M}}} \rmd s + t (\Mtt/(M\eta))^{1/2} \eqsp . }
\end{align}
We conclude upon using Gr\"{o}nwall's lemmma.
\end{proof}
